Prime+Probe 1, JavaScript 0: Overcoming Browser-based Side-Channel Defenses

The "eternal war in cache" has reached browsers, with multiple cache-based side-channel attacks and countermeasures being suggested. A common approach for countermeasures is to disable or restrict JavaScript features deemed essential for carrying out attacks. To assess the effectiveness of this approach, in this work we seek to identify those JavaScript features which are essential for carrying out a cache-based attack. We develop a sequence of attacks with progressively decreasing dependency on JavaScript features, culminating in the first browser-based side-channel attack which is constructed entirely from Cascading Style Sheets (CSS) and HTML, and works even when script execution is completely blocked. We then show that avoiding JavaScript features makes our techniques architecturally agnostic, resulting in microarchitectural website fingerprinting attacks that work across hardware platforms including Intel Core, AMD Ryzen, Samsung Exynos, and Apple M1 architectures. As a final contribution, we evaluate our techniques in hardened browser environments including the Tor browser, Deter-Fox (Cao el al., CCS 2017), and Chrome Zero (Schwartz et al., NDSS 2018). We confirm that none of these approaches completely defend against our attacks. We further argue that the protections of Chrome Zero need to be more comprehensively applied, and that the performance and user experience of Chrome Zero will be severely degraded if this approach is taken.

==> Makefile <==
# Generic paper Makefile
#
# For usage hints, "make help"
#
#  To create a LaTeX diff against the hg "tip" revision, use the target
#  "diff" (or "viewdiff").
#  To use a revision other than "tip", speciff DIFF=x on the 
#  make command line to choose the revision x.
#

# Verbosity
ifeq (${V},1)
Q:=
else
Q:=@
endif

.PHONY: all

BIBDIR     ?= /home/disy/lib/BibTeX:../../../bibtex:../bibtex
LaTeXEnv   = TEXINPUTS=".:/home/disy/lib/TeX:/home/disy/lib/ps:${TEXINPUTS}:"
BibTexEnv  = BIBINPUTS=".:${BIBDIR}:${BIBINPUTS}:"
BibFiles   = defs-abbrev,extra,combined,systems,fm,other

LaTeX      = ${LaTeXEnv} pdflatex -interaction=nonstopmode
LaTeXdiff  = ./tools/latexdiff
BibTeX     = ${BibTexEnv} bibtex
Fig2Eps    = fig2dev -L eps
Dia2Eps    = dia -t eps -e
AS         = $(shell which as)
CC         = $(shell which gcc)
GnuPlot	   = gnuplot
Inkscape   = $(shell which inkscape)
Eps2Pdf	   = epstopdf --outfile
PdfView	   = xpdf
Pdf2Ps	   = pdf2ps
RmCR       = tr -d '\r'
sed        = $(shell which sed)
#PdfView    = open -a preview
#PdfView    = acroread 
Lpr 	   = lpr
mv	   = mv
awk	   = awk
R	   = R

# Use either "report" or "paper", depending on the template.
# To add a further target, simply append the basename of the .tex file here
Targets    = pp0
SRCS = pp0.tex # methodology.tex


# CONFIGURATION OPTIONS
# =====================

# For ACM SIG camera ready submission. This will only work if Target
# is a single identifier. You should then be able to use the "camera" target,
# after setting CamRoot appropriately. Answer "no" for re-making references.bib
# Set CamRoot as the filename root per publisher's instructions.
# Should be <paperno>-<lastname-of-first-author>
CamRoot    = <paperno>-<last>
CamDir	   = cameraready

# Any other stuff that may be needed

# END CONFIGURATION OPTIONS
# =========================

Optional = $(addsuffix -diff, $(Targets))
All = $(Targets) $(Optional)
Diffopts= #--type=BWUNDERLINE #-c .latexdiffconfig --append-safecmd="Comment"

Gnuplot_Sources = $(wildcard figures/*.gnuplot)
Figures = $(Gnuplot_Sources:.gnuplot=.pdf)



Pdf = $(addsuffix .pdf, $(Targets))
Tex = $(addsuffix .tex, $(Targets))
Diff_Pdf = $(addsuffix .pdf, $(Optional))

.PHONY: FORCE

all: pdf
diff: diff_pdf
FORCE: pdf
ps: $(Ps)
pdf: $(Figures) Makefile $(Pdf)
diff_pdf: $(Figures) Makefile $(Diff_Pdf)

%.pdf: %.perf tools/bargraph.pl
	@echo $< '->' $@
	${Q} ${BarGraph} -pdf $< > $@

%.pdf: %.eps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

%.pdf: %.ps
	@echo $< '->' $@
	${Q} ${Eps2Pdf} $@ $<

#%.eps: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -E $@ > /dev/null 2>&1

#%.pdf: %.svg
#	@echo $< '->' $@
#	${Q} $(if ${Inkscape},,echo "You need inkscape installed to build $@" >&2; exit 1)
#	${Q} ${Inkscape} -f $< -D -z -A $@ > /dev/null 2>&1

# This target allows you to add figures which have the extension .c_pp that
# correspond to .c sources. Your .c sources can use the lines '/*<*/' and
# '/*>*/' to surround parts of the source you don't want shown in your PDF.
# This allows you to write a .c file that can be compile-checked here and then
# remove extraneous lines for display.
%.c_pp: %.c
	@echo $< '->' $@
	${Q}$(if ${CC},${CC} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.s_pp: %.s
	@echo $< '->' $@
	${Q}$(if ${AS},${AS} -c "$<" -o /dev/null,)
	${Q}${sed} -e '/\/\*<\*\//,/\/\*>\*\//d' "$<" >"$@"

%.eps: %.dia
	@echo $< '->' $@
	${Q} ${Dia2Eps} $@ $<

%.eps: %.fig
	@echo $< '->' $@
	${Q} ${Fig2Eps} $< $@

%.eps: %.gnuplot
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.pdf: %.gnuplotpdf
	@echo $< '->' $@
	${Q} ${GnuPlot} $<

%.eps: %.r
	@echo $< '->' $@
	${Q} ${R} --vanilla < $<

%.pdf: %.pdf-shipped
	cp $< $@

view: pdf
	${Q}for i in $(Pdf); do \
		$(PdfView) $$i & \
	done

viewdiff: diff
	${Q}for i in $(Diff_Pdf); do \
		$(PdfView) $$i & \
	done

print: pdf
	${Q}for i in $(Pdf); do \
		$(Lpr) $$i \
	done

clean:
	rm -f *.aux *.toc *.bbl *.blg *.dvi *.log *.pstex* *.eps *.cb *.brf \
		*.idx *.out *.ps *-diff.* *.mps .log *.diff pp0.pdf

help:
	@echo "Main targets: all diff camera view viewdiff print clean realclean tar"
	@echo "'make diff' will show changes to head revision"
	@echo "'make DIFF=<rev> diff' will show changes to revision <rev>"
	@echo "Avoid TeX \def with arguments, this breaks latexdiff (use \newcommand)"


##############################################################################

DIFF ?= tip

%-diff.dvi: %-diff.tex

%-diff.tex: %.tex FORCE
	@echo "====> Retrieving revision $(DIFF) of $<"
	hg cat -r $(DIFF) $<  > $(@:-diff.tex=-$(DIFF)-diff.tex)
	@echo "====> Creating diff of revision $(DIFF) of $<"
	$(LaTeXdiff) $(Diffopts) $(@:-diff.tex=-$(DIFF)-diff.tex) $< | \
	${RmCR} > $@

.PHONY: FORCE
FORCE:

# don't delete %.aux intermediates
.SECONDARY:

##############################################################################

Rerun = '(There were undefined (references|citations)|Rerun to get (cross-references|the bars) right)'
Rerun_Bib = 'No file.*\.bbl|Citation.*undefined'
Undefined = '((Reference|Citation).*undefined)|(Label.*multiply defined)'
Error = '^! '


pp0.pdf: pp0.tex  $(Figures) Makefile ${SRCS}
	${Q}if ! test -e pp0.bbl || test pp0.bib -nt pp0.bbl; then rm -f pp0.bbl; fi
	@echo "====> LaTeX first pass: $(<)"
	${Q}$(LaTeX) $< >.log || if egrep -q $(Error) pp0.log ; then cat .log; rm $@; false ; fi
	${Q}if egrep -q $(Rerun_Bib) pp0.log ; then echo "====> BibTex" && ( $(BibTeX) pp0 > .log || ( cat .log ; false ) ) && echo "====> LaTeX BibTeX pass" && $(LaTeX) >.log $< || if egrep -q $(Error) pp0.log ; then cat .log; rm $@; false ; fi ; fi
	${Q}if egrep -q $(Rerun) pp0.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) pp0.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if egrep -q $(Rerun) pp0.log ; then echo "====> LaTeX rerun" && $(LaTeX) >.log $<; fi
	${Q}if [ -a .NeedGS ]; then gs -dSAFER -dBATCH -dNOPAUSE  -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $@; mv tmp.pdf $@; fi
	@echo "====> Undefined references and citations in $(<):"
	@egrep -i $(Undefined) pp0.log || echo "None."
	@echo "====> Dimensions:"
	@grep "dimension:" pp0.log || echo "None."

##############################################################################
# Generate a list of FIXMEs 
fixmes: 
	${Q}for i in $(Tex); do \
		echo "FIXMEs in $$i:"; \
		nl -b a $$i | grep "FIXME{" | nl -b a; \
		echo -n "Total FIXMES: " && grep "FIXME{" $$i | wc -l; \
		echo; \
	done

usb.pdf: dtrt.sty

